Few-Shot Meta Learning for Recognizing Facial Phenotypes of Genetic Disorders

Computer vision-based methods have valuable use cases in precision medicine, and recognizing facial phenotypes of genetic disorders is one of them. Many genetic disorders are known to affect faces' visual appearance and geometry. Automated classification and similarity retrieval aid physicians in decision-making to diagnose possible genetic conditions as early as possible. Previous work has addressed the problem as a classification problem and used deep learning methods. The challenging issue in practice is the sparse label distribution and huge class imbalances across categories. Furthermore, most disorders have few labeled samples in training sets, making representation learning and generalization essential to acquiring a reliable feature descriptor. In this study, we used a facial recognition model trained on a large corpus of healthy individuals as a pre-task and transferred it to facial phenotype recognition. Furthermore, we created simple baselines of few-shot meta-learning methods to improve our base feature descriptor. Our quantitative results on GestaltMatcher Database show that our CNN baseline surpasses previous works, including GestaltMatcher, and few-shot meta-learning strategies improve retrieval performance in frequent and rare classes.

==> arXiv 2210.12705 - LaTeX source/figures/colors.tex <==
\definecolor{gray1}{rgb}{0.7, 0.7, 0.7}
\definecolor{gray2}{rgb}{0.8, 0.8, 0.8}
\definecolor{gray3}{rgb}{0.9, 0.9, 0.9}
\definecolor{red1}{rgb}{0.9, 0.4, 0.4}
\definecolor{red2}{rgb}{0.8, 0.3, 0.3}
\definecolor{red3}{rgb}{0.7, 0.2, 0.2}
\definecolor{green1}{rgb}{0.4, 0.7, 0.4}
\definecolor{green2}{rgb}{0.5, 0.8, 0.5}
\definecolor{green3}{rgb}{0.6, 0.9, 0.6}
\definecolor{blue1}{rgb}{0.5, 0.5, 0.7}
\definecolor{blue2}{rgb}{0.6, 0.6, 0.8}
\definecolor{blue3}{rgb}{0.7, 0.7, 0.9}
\definecolor{yellow1}{rgb}{1, 0.8, 0.6}
\definecolor{yellow2}{rgb}{1, 0.9, 0.6}
\definecolor{yellow3}{rgb}{1, 1, 0.6}

% Colors for rare
\definecolor{color0}{rgb}{1.0,0.1,0.1}
\definecolor{color1}{rgb}{1.0,0.3,0.3}
\definecolor{color2}{rgb}{1.0,0.5,0.5}
\definecolor{color3}{rgb}{1.0,0.7,0.7}
% Colors for freq
\definecolor{color4}{rgb}{0.1,0.1,1.0}
\definecolor{color5}{rgb}{0.3,0.3,1.0}
\definecolor{color6}{rgb}{0.5,0.5,1.0}
\definecolor{color7}{rgb}{0.7,0.7,1.0}

==> arXiv 2210.12705 - LaTeX source/figures/rare_vs_freq_line_chart.tex <==
% This file was created by tikzplotlib v0.9.4.
\begin{tikzpicture}[scale=0.65,every node/.style={scale=1.3}]

\begin{axis}[
legend cell align={left},
legend style={fill opacity=0.8, draw opacity=1, text opacity=1, at={(1.6,0.1)}, anchor=south east, draw=white!80!black},
tick align=outside,
tick pos=left,
x grid style={white!69.0196078431373!black},
xlabel={Epoch},
xmajorgrids,
xmin=0, xmax=9,
xtick style={color=black},
y grid style={white!69.0196078431373!black},
ylabel={Accuracy},
ymajorgrids,
ymin=0, ymax=1,
ytick style={color=black}
]
% Best epoch on validation accuracy
\draw [dashed] (3,-1) -- (3,1);
% Rare - Top-1
\addplot [only marks, mark=*, draw=color0, fill=color0, colormap/viridis]
table{%
x                      y
0 0.35280
1 0.34300
2 0.33480
3 0.32420
4 0.31590
5 0.29190
6 0.28280
7 0.25650
8 0.24500
9 0.23480
};
\addlegendentry{Rare - Top-1}
\addplot [semithick, color0, forget plot]
table {%
0 0.35280
1 0.34300
2 0.33480
3 0.32420
4 0.31590
5 0.29190
6 0.28280
7 0.25650
8 0.24500
9 0.23480
};

% Rare - Top-5
\addplot [only marks, mark=*, draw=color1, fill=color1, colormap/viridis]
table{%
x                      y
0 0.50900
1 0.50770
2 0.50980
3 0.50210
4 0.47610
5 0.46750
6 0.45030
7 0.43530
8 0.40860
9 0.39910
};
\addlegendentry{Rare - Top-5}
\addplot [semithick, color1, forget plot]
table {%
0 0.50900
1 0.50770
2 0.50980
3 0.50210
4 0.47610
5 0.46750
6 0.45030
7 0.43530
8 0.40860
9 0.39910
};

% Rare - Top-10
\addplot [only marks, mark=*, draw=color2, fill=color2, colormap/viridis]
table{%
x                      y
0 0.59240
1 0.58950
2 0.59810
3 0.58810
4 0.56920
5 0.55570
6 0.53980
7 0.52060
8 0.50170
9 0.48500
};
\addlegendentry{Rare - Top-10}
\addplot [semithick, color2, forget plot]
table {%
0 0.59240
1 0.58950
2 0.59810
3 0.58810
4 0.56920
5 0.55570
6 0.53980
7 0.52060
8 0.50170
9 0.48500
};

% Rare - Top-30
\addplot [only marks, mark=*, draw=color3, fill=color3, colormap/viridis]
table{%
x                      y
0 0.72320
1 0.72960
2 0.72210
3 0.72040
4 0.71510
5 0.69730
6 0.68220
7 0.66440
8 0.64600
9 0.62380
};
\addlegendentry{Rare - Top-30}
\addplot [semithick, color3, forget plot]
table {%
0 0.72320
1 0.72960
2 0.72210
3 0.72040
4 0.71510
5 0.69730
6 0.68220
7 0.66440
8 0.64600
9 0.62380
};


% Frequent - Top-1
\addplot [only marks, mark=*, draw=color4, fill=color4, colormap/viridis]
table{%
x                      y
0 0.42159
1 0.41484
2 0.42327
3 0.43339
4 0.45025
5 0.45363
6 0.44351
7 0.45363
8 0.44519
9 0.43845
};
\addlegendentry{Frequent - Top-1}
\addplot [semithick, color4, forget plot]
table {%
0 0.42159
1 0.41484
2 0.42327
3 0.43339
4 0.45025
5 0.45363
6 0.44351
7 0.45363
8 0.44519
9 0.43845
};

% Frequent - Top-5
\addplot [only marks, mark=*, draw=color5, fill=color5, colormap/viridis]
table{%
x                      y
0 0.65936
1 0.65599
2 0.67285
3 0.66610
4 0.66273
5 0.65261
6 0.64081
7 0.63912
8 0.63238
9 0.62563
};
\addlegendentry{Frequent - Top-5}
\addplot [semithick, color5, forget plot]
table {%
0 0.65936
1 0.65599
2 0.67285
3 0.66610
4 0.66273
5 0.65261
6 0.64081
7 0.63912
8 0.63238
9 0.62563
};

% Frequent - Top-10
\addplot [only marks, mark=*, draw=color6, fill=color6, colormap/viridis]
table{%
x                      y
0 0.74874
1 0.76728
2 0.76728
3 0.76897
4 0.74368
5 0.74368
6 0.70658
7 0.70995
8 0.70489
9 0.67454
};
\addlegendentry{Frequent - Top-10}
\addplot [semithick, color6, forget plot]
table {%
0 0.74874
1 0.76728
2 0.76728
3 0.76897
4 0.74368
5 0.74368
6 0.70658
7 0.70995
8 0.70489
9 0.67454
};

% Frequent - Top-30
\addplot [only marks, mark=*, draw=color7, fill=color7, colormap/viridis]
table{%
x                      y
0 0.86003
1 0.87521
2 0.85835
3 0.85497
4 0.86172
5 0.84654
6 0.84148
7 0.81282
8 0.78752
9 0.76391
};
\addlegendentry{Frequent - Top-30}
\addplot [semithick, color7, forget plot]
table {%
0 0.86003
1 0.87521
2 0.85835
3 0.85497
4 0.86172
5 0.84654
6 0.84148
7 0.81282
8 0.78752
9 0.76391
};
\end{axis}

\end{tikzpicture}


==> figures/rare_vs_freq_line_chart.tex <==
% This file was created by tikzplotlib v0.9.4.
\begin{tikzpicture}[scale=0.65,every node/.style={scale=1.3}]

\begin{axis}[
legend cell align={left},
legend style={fill opacity=0.8, draw opacity=1, text opacity=1, at={(1.6,0.1)}, anchor=south east, draw=white!80!black},
tick align=outside,
tick pos=left,
x grid style={white!69.0196078431373!black},
xlabel={Epoch},
xmajorgrids,
xmin=0, xmax=9,
xtick style={color=black},
y grid style={white!69.0196078431373!black},
ylabel={Accuracy},
ymajorgrids,
ymin=0, ymax=1,
ytick style={color=black}
]
% Best epoch on validation accuracy
\draw [dashed] (3,-1) -- (3,1);
% Rare - Top-1
\addplot [only marks, mark=*, draw=color0, fill=color0, colormap/viridis]
table{%
x                      y
0 0.35280
1 0.34300
2 0.33480
3 0.32420
4 0.31590
5 0.29190
6 0.28280
7 0.25650
8 0.24500
9 0.23480
};
\addlegendentry{Rare - Top-1}
\addplot [semithick, color0, forget plot]
table {%
0 0.35280
1 0.34300
2 0.33480
3 0.32420
4 0.31590
5 0.29190
6 0.28280
7 0.25650
8 0.24500
9 0.23480
};

% Rare - Top-5
\addplot [only marks, mark=*, draw=color1, fill=color1, colormap/viridis]
table{%
x                      y
0 0.50900
1 0.50770
2 0.50980
3 0.50210
4 0.47610
5 0.46750
6 0.45030
7 0.43530
8 0.40860
9 0.39910
};
\addlegendentry{Rare - Top-5}
\addplot [semithick, color1, forget plot]
table {%
0 0.50900
1 0.50770
2 0.50980
3 0.50210
4 0.47610
5 0.46750
6 0.45030
7 0.43530
8 0.40860
9 0.39910
};

% Rare - Top-10
\addplot [only marks, mark=*, draw=color2, fill=color2, colormap/viridis]
table{%
x                      y
0 0.59240
1 0.58950
2 0.59810
3 0.58810
4 0.56920
5 0.55570
6 0.53980
7 0.52060
8 0.50170
9 0.48500
};
\addlegendentry{Rare - Top-10}
\addplot [semithick, color2, forget plot]
table {%
0 0.59240
1 0.58950
2 0.59810
3 0.58810
4 0.56920
5 0.55570
6 0.53980
7 0.52060
8 0.50170
9 0.48500
};

% Rare - Top-30
\addplot [only marks, mark=*, draw=color3, fill=color3, colormap/viridis]
table{%
x                      y
0 0.72320
1 0.72960
2 0.72210
3 0.72040
4 0.71510
5 0.69730
6 0.68220
7 0.66440
8 0.64600
9 0.62380
};
\addlegendentry{Rare - Top-30}
\addplot [semithick, color3, forget plot]
table {%
0 0.72320
1 0.72960
2 0.72210
3 0.72040
4 0.71510
5 0.69730
6 0.68220
7 0.66440
8 0.64600
9 0.62380
};


% Frequent - Top-1
\addplot [only marks, mark=*, draw=color4, fill=color4, colormap/viridis]
table{%
x                      y
0 0.42159
1 0.41484
2 0.42327
3 0.43339
4 0.45025
5 0.45363
6 0.44351
7 0.45363
8 0.44519
9 0.43845
};
\addlegendentry{Frequent - Top-1}
\addplot [semithick, color4, forget plot]
table {%
0 0.42159
1 0.41484
2 0.42327
3 0.43339
4 0.45025
5 0.45363
6 0.44351
7 0.45363
8 0.44519
9 0.43845
};

% Frequent - Top-5
\addplot [only marks, mark=*, draw=color5, fill=color5, colormap/viridis]
table{%
x                      y
0 0.65936
1 0.65599
2 0.67285
3 0.66610
4 0.66273
5 0.65261
6 0.64081
7 0.63912
8 0.63238
9 0.62563
};
\addlegendentry{Frequent - Top-5}
\addplot [semithick, color5, forget plot]
table {%
0 0.65936
1 0.65599
2 0.67285
3 0.66610
4 0.66273
5 0.65261
6 0.64081
7 0.63912
8 0.63238
9 0.62563
};

% Frequent - Top-10
\addplot [only marks, mark=*, draw=color6, fill=color6, colormap/viridis]
table{%
x                      y
0 0.74874
1 0.76728
2 0.76728
3 0.76897
4 0.74368
5 0.74368
6 0.70658
7 0.70995
8 0.70489
9 0.67454
};
\addlegendentry{Frequent - Top-10}
\addplot [semithick, color6, forget plot]
table {%
0 0.74874
1 0.76728
2 0.76728
3 0.76897
4 0.74368
5 0.74368
6 0.70658
7 0.70995
8 0.70489
9 0.67454
};

% Frequent - Top-30
\addplot [only marks, mark=*, draw=color7, fill=color7, colormap/viridis]
table{%
x                      y
0 0.86003
1 0.87521
2 0.85835
3 0.85497
4 0.86172
5 0.84654
6 0.84148
7 0.81282
8 0.78752
9 0.76391
};
\addlegendentry{Frequent - Top-30}
\addplot [semithick, color7, forget plot]
table {%
0 0.86003
1 0.87521
2 0.85835
3 0.85497
4 0.86172
5 0.84654
6 0.84148
7 0.81282
8 0.78752
9 0.76391
};
\end{axis}

\end{tikzpicture}

